Mapping distributional to model-theoretic semantic spaces: a baseline

Word embeddings have been shown to be useful across state-of-the-art systems in many natural language processing tasks, ranging from question answering systems to dependency parsing. (Herbelot and Vecchi, 2015) explored word embeddings and their utility for modeling language semantics. In particular, they presented an approach to automatically map a standard distributional semantic space onto a set-theoretic model using partial least squares regression. We show in this paper that a simple baseline achieves a +51% relative improvement compared to their model on one of the two datasets they used, and yields competitive results on the second dataset.

==> introduction.tex <==
\section{Introduction and related work}

Artificial neural networks (ANNs) have recently shown state-of-the-art results on various NLP tasks including 
language modeling~\cite{mikolov2010recurrent},  named entity recognition~\cite{collobert2011natural,lample2016neural,labeau-loser-allauzen:2015:EMNLP}, text classification~\cite{socher2013recursive,kim2014convolutional,blunsom2014convolutional,lee2016sequential}, question answering~\cite{weston2015towards,wang-nyberg:2015:ACL-IJCNLP}, and machine translation~\cite{bahdanau2014neural,tamura2014recurrent}.

Using ANNs for NLP tasks do not require manually engineered features.
However, ANNs have hyperparameters that need to be tuned in order to achieve the best results. The hyperparameters of ANNs may define either its learning process (e.g., learning rate or mini-batch size) or its architecture (e.g., number of hidden units or layers). ANNs commonly contain over ten hyperparameters~\cite{bengio2012practical}, which makes it challenging to optimize.

The hyperparameters are typically optimized using manual, grid or random search~\cite{bergstra2012random}.
 Manual search requires human experts while random and grid search are computationally expensive. 


 More systematic approaches such as Bayesian optimization with Gaussian process~(GP) \cite{williams2006gaussian} have been shown to be effective in tuning some machine learning models~\cite{NIPS2011_4443,NIPS2012_4522}. 
 
However, most ANN-based NLP works rely on basic heuristics such as manual, random or grid search, and sometimes do not even optimize hyperparameters. 
In this work, we investigate the application of GP to optimize ANN hyperparameters using the dialog act classification task~\cite{stolcke2000dialogue}, whose goal is to assign a dialog act to each utterance.
\hspace{-0.02cm}Optimizing hyperparameters with GP yields state-of-the-art results on two datasets, and most importantly reduces the computational time by a factor of 4 compared to a random search.



